PARIKSHA: A Large-Scale Investigation of Human-LLM Evaluator Agreement on Multilingual and Multi-Cultural Data

Evaluation of multilingual Large Language Models (LLMs) is challenging due to a variety of factors -- the lack of benchmarks with sufficient linguistic diversity, contamination of popular benchmarks into LLM pre-training data and the lack of local, cultural nuances in translated benchmarks. In this work, we study human and LLM-based evaluation in a multilingual, multi-cultural setting. We evaluate 30 models across 10 Indic languages by conducting 90K human evaluations and 30K LLM-based evaluations and find that models such as GPT-4o and Llama-3 70B consistently perform best for most Indic languages. We build leaderboards for two evaluation settings - pairwise comparison and direct assessment and analyze the agreement between humans and LLMs. We find that humans and LLMs agree fairly well in the pairwise setting but the agreement drops for direct assessment evaluation especially for languages such as Bengali and Odia. We also check for various biases in human and LLM-based evaluation and find evidence of self-bias in the GPT-based evaluator. Our work presents a significant step towards scaling up multilingual evaluation of LLMs.

==> content/acknowledgements.tex <==
\section{Acknowledgements}
\label{sec:acknowledgements}
We thank the \textsc{Karya} team, as well as the workers and annotators, whose efforts made the annotation work possible. We extend our gratitude to the native speakers from Microsoft Research India who helped us curate language-specific prompts. Lastly, we also acknowledge the valuable input provided by our partners and collaborators from \textit{Glocal Evaluation of Models (GEM)}\footnote{\url{https://peopleplus.ai/leaderboard}} and People+AI in shaping this work.


